AutoML to Date and Beyond: Challenges and Opportunities

As big data becomes ubiquitous across domains, and more and more stakeholders aspire to make the most of their data, demand for machine learning tools has spurred researchers to explore the possibilities of automated machine learning (AutoML). AutoML tools aim to make machine learning accessible for non-machine learning experts (domain experts), to improve the efficiency of machine learning, and to accelerate machine learning research. But although automation and efficiency are among AutoML's main selling points, the process still requires human involvement at a number of vital steps, including understanding the attributes of domain-specific data, defining prediction problems, creating a suitable training data set, and selecting a promising machine learning technique. These steps often require a prolonged back-and-forth that makes this process inefficient for domain experts and data scientists alike, and keeps so-called AutoML systems from being truly automatic. In this review article, we introduce a new classification system for AutoML systems, using a seven-tiered schematic to distinguish these systems based on their level of autonomy. We begin by describing what an end-to-end machine learning pipeline actually looks like, and which subtasks of the machine learning pipeline have been automated so far. We highlight those subtasks which are still done manually - generally by a data scientist - and explain how this limits domain experts' access to machine learning. Next, we introduce our novel level-based taxonomy for AutoML systems and define each level according to the scope of automation support provided. Finally, we lay out a roadmap for the future, pinpointing the research required to further automate the end-to-end machine learning pipeline and discussing important challenges that stand in the way of this ambitious goal.

==> Challenges.tex <==
\section{Challenges}\label{sec:Challenges}
 Below we provide a brief summary of the technical challenges:


\begin{enumerate}
    \item How to computationally generate a wide range of prediction task? Can we devise a general language to express prediction tasks? What would be the variable types and operators of that language?
    
    \item How do we interpret the prediction task language expressions into more human readable format?
    
    \item How do we know if a particular prediction task is valid?
    
    \item How to model the ranking function of the recommender system? Given a corpus of Big Data, what is the ideal objective function which the recommender system should optimize for. How to make the recommender system more efficient and scalable?
    
    \item How to evaluate the usefulness of a prediction task? What does usefulness really mean in this context? In other words, how do we evaluate the performance of a prediction-task recommender system?
    
    \item How can we improve the recommender system by actively learning from feedback provided by the user?
\end{enumerate}


To study the feasibility of converting the hypothetical VDS into a real system, we conducted an exploratory case-study with three different real world data sets from Kaggle to understand how VDS can be materialized in practical scenario. This also helped us in understanding the aforementioned challenges in greater detail.  The following sections provide more details on the data sets explored and highlights the challenges needs to be addressed to design a fully functional VDS.


\section{An Exploratory Case-Study}\label{sec:case}
\begin{table}[tb]

\tbl{Dataset details\label{tab:columns}}
    {\begin{tabularx}{\linewidth}{@{\extracolsep{\fill}}lX}\toprule
    Dataset & Column Nane and Meanings \\\midrule
    Chicago          & date, hour (date and hour of the trip)                                                                                                   \\
    Bicycle          & user\_type (either one-day pass or annual subscription)                                                                                  \\
                     & gender                                                                                                                                   \\
                     & trip\_duration, temperature                                                                                                              \\
                     & from\_station\_id, to\_station\_id                                                                                                       \\
                     & dpcapacity\_st, dpcapacity\_ed (number of docks in origin and destination stations)                      \\\midrule
    Flight           & date, day\_of\_week                                                                                                                      \\
    Delay            & airline, flight\_number, tail\_number                                                                                                    \\
                     & origin\_airport, destination\_airport                                                                                                    \\
                     & scheduled\_departure\_hour                                                                                                               \\
                     & scheduled\_time, elapsed\_time (the scheduled trip time and the actual time)                                                             \\
                     & departure\_delay, arrival\_delay (the departure delay and arrival delay in minute)                                                       \\
                     & cancelled, cancelation\_reason (whether the flight is canceled and categorical cancelation reason)                                       \\
                     & air\_system\_delay, security\_delay, airline\_delay, late\_aircraft\_delay, weather\_delay (delay caused by different reasons in minute) \\\midrule
    YouTube          & trending\_date (the date when the video is trending)                                                                                     \\
    Trending         & channel\_title (the title of a youtube channel)                                                                                          \\
                     & category\_id (the category of a video)                                                                                                   \\
                     & views, likes, dislikes, comment\_count (the number of views, likes, dislikes and comment counts when the video starts trending)          \\\bottomrule
    \end{tabularx}}
\end{table}



We picked $3$ event-driven time series datasets from Kaggle and generate prediction problems on them. \textbf{Chicago Bicycle}\footnote{https://www.kaggle.com/yingwurenjian/chicago-divvy-bicycle-sharing-data} records the use of shared bicycles in Chicago between 2014 and 2017. \textbf{Flight Delay}\footnote{https://www.kaggle.com/usdot/flight-delays} is the 2015 flight records in US. \textbf{YouTube Trending}\footnote{https://www.kaggle.com/datasnaek/youtube-new} records trending YouTube videos between 2017 and 2018. Each dataset has a time column. We pick the time column, entity columns, numerical columns, and categorical columns, while removing unsupported columns like sets or natural language. Table \ref{tab:columns} shows columns we use to generate prediction problems and Table \ref{tab:ncol} shows the number of columns in each dataset.


\begin{table}[htb]
    \tbl{Number of entity columns, categorical columns and numerical columns in each dataset\label{tab:ncol}}
    {\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lccc}\toprule
    Dataset          & \#Entity & \#Categorical & \#Numerical \\\midrule
    Chicago Bicycle  & 2        & 3             & 4           \\
    Flight Delay     & 4        & 4             & 10          \\
    YouTube Trending & 1        & 1             & 4          \\\bottomrule
    \end{tabular*}}
\end{table}





We now briefly discuss the challenges of designing VDS in light of the three data sets mentioned above:


\section{Formalization of prediction task search}
To enable search through prediction tasks, we imagine two distinct research threads. First, developing a formal specification of the prediction task, and second optimizing the search process by learning from human data scientists. Each of these components present unique challenges that we will briefly describe this paper. We envision that fully solving these challenges, would require a line of inquiry and research and present motivating examples for the community to jointly pursue them. 

\subsection{\bf Formalization of a prediction task} 
The first and most important challenge in designing \vds is to design a generic language that can express many different prediction tasks. We begin by noticing that in a variety of prediction tasks across multiple domains, a prediction task is usually characterized by: an outcome function $f(.)$, a window called \pw over which this outcome is calculated, the time into the future one wishes to predict this outcome, called \lead. Several other parameters control the way data is prepared for machine learning and how the eventual model will be made operational. Consider the following examples over our datasets. 

\begin{exmp}

\end{exmp}

\begin{exmp}
\end{exmp}

Abstracting away the \pw, \lead and other parameters from the $f(.)$ allows us to focus on where the most important translation from human intuition to problem specification happens, which is the definition of the outcome function $f(.)$. Human data scientists translate an abstract goal of predict \textit{customer engagement} to a \textit{computable quantity} that could be predicted. For example, engagement by one definition could be quantified as ``\textit{the number of visits a customer has to the website during a week}''. Here the outcome function is ``\textit{number of visits to the website''} and the \pw is one week. Thus a prediction task in this paper is defined as 
\begin{defn}
\end{defn}
\kedit{}{We would have to use this section to also provide an argument as to how this different than a standard analytic query. it maybe not any different than a standard data analytic query, but it is in a different context}

Thus to develop \vds one would need a language in which the prediction tasks could be specified. 

As with any language, one needs to define variable types as well as operators/functions to specify the Language for VDS. Let us call this language ``PeTEL'', which stands for ``prediction task expression Language''. 


The variable types of ``PeTEL'' can be as simple as integers, real-valued numbers, categorical attributes or they can be complex variables like entities, events etc. The details of these types will of-course vary based on the implementations. On the other hand, the operators will depend on the specific variable types. Some basic  operators can be Filter operator (equal filter, greater than filter etc.), Aggregation operators (count, sum, average etc.), Smoothing operators (to handle missing values in the data). Table~\ref{table:op} shows some example operators of VDS and their supported types.

\begin{table}[htb]
    \tbl{Operators\label{table:op}}
    {\begin{tabular}{p{1.00in}p{2.00in}p{1.00in}}
            \toprule
            Operation Set & Supported Ops & Supported Types \\\midrule
            Filter & \texttt{all\_fil} & None\\
            $\mathbf{O}_f$    & \texttt{greater\_fil}, \texttt{less\_fil} & Numerical\\
            & \texttt{eq\_fil}, \texttt{neq\_fil} & Categorical/Entity\\\midrule
            Aggregation & \texttt{count\_agg} & None\\
            $\mathbf{O}_g$    & \texttt{sum\_agg}, \texttt{avg\_agg}, & Numerical \\
               & \texttt{min\_agg}, \texttt{max\_agg} & Numerical \\
            & \texttt{majority\_agg} & Categorical/Entity \\
            \bottomrule
        \end{tabular}}
\end{table}





\subsubsection{\bf Interpretability of a Task:}
The next challenge to materialize VDS is how to interpret the \emph{PeTEL} expression of a prediction task to a human readable language. For example, think about the following PeTEL expression: \\

$<$AIRLINE$>$ [eq\_filter($<$CANCELLATION\_REASON,``bad\_weather''$>$),\\majority\_agg($<$DESTINATION\_AIRPORT$>$)]\\

Although people with basic knowledge about structured query language may understand the meaning behind this expression, it is very hard for people with other background to dig out the actual prediction task expressed in this PeTEL expression. However, if VDS translates the PeTEL expression into the following natural language form: ``For each airline, Predict which destination airport has the most number of flights canceled because of weather tomorrow'', it becomes clear to the user which prediction task is being proposed by VDS. Thus, translating PeTEL expressions into human readable language is a core 
challenge which needs to be addressed in order to make VDS appealing to a wider range of audience.





\subsubsection{\bf Validity of a Task:}
Another challenge for VDS is to check the validity of a prediction task. Given that \emph{PeTEL} can output many different prediction tasks through combinations of operators and variables, not all combination would yield a valid task. In fact, a large portion of them would be invalid. For example, \emph{PeTEL} can propose a prediction problem for the Flight delay data set as the following: ``For each airline, predict how many flights tomorrow will arrive at the destination before it departs''. \emph{PeTEL} expression for this prediction language can be something like this:\\

$<$AIRLINE$>$ [less\_filter($<$ARRIVAL\_TIME$>$,$<$DEPARTURE\_TIME$>$),count\_agg(None)]\\

where a less\_filter is applied first to check if the ARRIVAL\_TIME is less than the DEPARTURE\_TIME and then, a count operation is performed over the filtered records after grouping them by Airlines. Although this is a syntactically correct task, it is not semantically meaningful. Thus, a really important challenge for VDS to solve is to validate a proposed task.








\subsection{Prediction Opportunity Exploration (POE)}
\subsubsection{\bf Efficiency and Scalability:}
As VDS is expected to explore and evaluate a wide range of tasks, Efficiency and Scalability is another big issue to resolve. Given that PeTEL has to deal with many different attributes and operator types and the search space is exponential in the number of attributes as well as the number of operators, VDS has to find out efficient and Scalable alternatives through heuristics and approximation techniques to explore and evaluate a wide range of tasks. Also, there are a wide variety of feature engineering and machine learning models that can be explored for each prediction task. All these different pathways demand a huge computational effort which is very challenging. The major goal of addressing this challenge is to constrain the search space and reduce the computational requirement to a feasible amount.






\subsection{Result Summarizing and Recommendations (RSR)}
\subsubsection{\bf Recommending Useful Tasks}
As a prediction task recommender system, a major challenge for VDS is to filter out tasks that are not useful. In the context of VDS, the ``usefulness'' of a task is highly dependent on the domain expert / business leader it is interacting with. Thus, quickly learning an effective recommender system that can serve the users need is critical to the usability of VDS. In other words, how can VDS quickly rank a set of prediction tasks in terms of their usefulness and recommend the most useful tasks to the user? The core technical challenge that needs to be solved here is to design a ranker for the recommender system, which in turn, means to design an effective ``usefulness'' metric to evaluate a prediction task. 


Through initial experiments conducted on the three data sets mentioned in section~\ref{sec:case}, we present some example recommended tasks in Table~\ref{table:example} that were found through manual inspection. The details of this experiment is beyond the scope of this position paper, whose primary focus is to highlight the limitations of the current machine learning pipeline in practice and introduce the vision of VDS to address it.




\begin{table*}[htb]
\tbl{Top rated prediction problems on Chicago Bicycle, Flight Delay, and YouTube Trending dataset. O is the structural representation of the problem, including entity and a sequence of operations. G is the generated description of the problem. H is the human interpretation of the problem. \label{table:example}}
    {
\begin{tabularx}{\linewidth}{|X|}\hline
\textbf{Chicago Bicycle} \\
O: $<$from\_station\_id$>$ [all\_filter(None), count\_agg(None)]\\
G: For each $<$from\_station\_id$>$ predict the number of records\\
N: Predict how many trips will start from this station tomorrow.\\\hline

O: $<$from\_station\_id$>$ [eq\_filter($<$usertype$>$), count\_agg(None)]\\
G: For each $<$from\_station\_id$>$ predict the number of records with $<$usertype$>$ equal to \_\_\\
N: Predict how many riders without an annual subscription will start a trip from this station tomorrow.\\\hline

O: $<$from\_station\_id$>$ [less\_filter($<$temperature$>$), majority\_agg(to\_station\_id)]\\
G: For each $<$from\_station\_id$>$ predict the majority of $<$to\_station\_id$>$ in all related records with $<$temperature$>$ less than \_\_\\
N: Predict where do people usually go from this station next week when temperature is very low.\\\hline

O: $<$from\_station\_id$>$ [eq\_filter($<$gender$>$), count\_agg(None)]\\
G: For each $<$from\_station\_id$>$ predict the number of records with $<$gender$>$ equal to \_\_\\
N: Predict how many females will start a trip from this station tomorrow.\\\hline 

O: $<$from\_station\_id$>$ [greater\_filter($<$usertype$>$), average\_agg(None)]\\
G: For each $<$from\_station\_id$>$ predict the average of $<$tripduration$>$ in all related records with $<$temperature$>$ greater than \_\_\\
N: Predict how long on average will each user ride tomorrow when temprature is very high.\\\hline\hline

\textbf{Flight Delay} \\
O: $<$AIRLINE$>$ [all\_filter(None), max\_agg($<$ARRIVAL\_DELAY$>$)]\\
G: For each $<$AIRLINE$>$ predict the maximum of $<$ARRIVAL\_DELAY$>$ in all related records\\
N: Predict the delayed time for each airline's most delayed flight tomorrow.\\\hline

O: $<$AIRLINE$>$ [less\_fileter($<$ELAPSED\_TIME$>$, sum\_agg($<$AIRLINE\_DELAY$>$))]\\
G: For each $<$AIRLINE$>$ predict the total $<$AIRLINE\_DELAY$>$ in all related records with $<$ELAPSED\_TIME$>$ less than \_\_\\
N: Predict the total flight delay tomorrow for each airline's short haul flights.\\\hline

O: $<$AIRLINE$>$ [greater\_filter($<$AIRLINE\_DELAY$>$), majority\_agg($<$DESTINATION\_AIRPORT$>$)]\\
G: For each $<$AIRLINE$>$ predict the majority of $<$DESTINATION\_AIRPORT$>$ in all related records with $<$AIRLINE\_DELAY$>$ greater than \_\_\\
N: For each airline, predict which destination is the most likely to have delays caused by the airline itself. \\\hline

O: $<$ORIGIN\_AIRPORT$>$ [greater\_filter($<$DEPARTURE\_DELAY$>$), majority\_agg(None)]\\
G: For each $<$ORIGIN\_AIRPORT$>$ predict the number of records with $<$DEPARTURE\_DELAY$>$ greater than \_\_\\
N: Predict how many flights depart from this airport will be delayed more than 1 hour. \\\hline

O: $<$AIRLINE$>$ [eq\_filter($<$CANCELLATION\_REASON$>$), majority\_agg($<$DESTINATION\_AIRPORT$>$)]\\
G: For each $<$AIRLINE$>$ predict the majority of $<$DESTINATION\_AIRPORT$>$ in all related records with $<$CANCELLATION\_REASON$>$ equal to \_\_\\
N: Predict which destination airport has the most number of flights canceled because of weather tomorrow. \\
\hline\hline
\textbf{YouTube} \\
O: $<$channel\_title$>$, [all\_filter(None), count\_agg(None)]\\
G: For each $<$channel\_title$>$ predict the number of records.\\
N: Can you predict how many videos from this channel will be selected as trending video next month?\\\hline

O: $<$channel\_title$>$, [all\_filter(None), minimum\_agg($<$views$>$)]\\
G: For each $<$channel\_title$>$ predict the minimum of $<$views$>$ in all related records.\\
H: Can you predict the lowest view among all the trending videos from this channel next month? \\\hline

O: $<$channel\_title$>$, [less\_filter($<$view$>$), count\_agg(None)]\\
G: For each $<$channel\_title$>$ predict the number of records with $<$likes$>$ less than \_\_\\
H: Among all the videos selected as trending videos from this channel, can you predict how many of them have less than 1k views?\\\hline

O: $<$category\_id$>$, [all\_filter(None), sum\_agg($<$comment\_count$>$)]\\
G: For each $<$category\_id$>$ predict the total $<$comment\_count$>$ in all related records\\
H: Can you predict how many comment will all sport trending videos get tomorrow?\\\hline

O: $<$channel\_title$>$, [eq\_filter($<$category\_id$>$), sum\_agg($<$views$>$)]\\
G: For each $<$channel\_title$>$ predict the total $<$views$>$ in all related records with $<$category\_id$>$ equal to \_\_\\
H: How many views will the political trending videos from this channel get tomorrow?\\
\hline
\end{tabularx}}
\end{table*}





\subsubsection{\bf Feedback and Revision of Recommender system :} The remaining challenge for materializing VDS is to revise the recommendation model by actively learning from user feedback. VDS can initially recommend a set of tasks that are highly scored by the recommender system and ask the user to label tasks as ``useful'' and ``not-useful''. By looking at these feedback, VDS can learn about the users preference and revise the recommendation model to accommodate them. This recommendation-modification loop can continue until the user is satisfied or completely hopeless with the recommendation. Another interesting challenge is to transfer the knowledge learned by interacting with users from one domain to another domain and see how users from another domain reacts to such recommendations.

==> Intro_v1.tex <==



\section{Big Data and Machine Learning}\label{sec:intro}
The twenty-first century has seen a massive increase in web-based systems, and this has itself resulted in the generation of ``big data.'' Companies across all domains and applications are newly focused on exploiting this data in order to improve their products and services and understand their users' needs. The rapid growth of machine learning (ML) infrastructure and high performance computing have significantly contributed to this process. Business entities are hiring more and more data scientists (5X growth) and ML engineers (12X growth) in order to better make sense of their data \cite{linkedin}, and industry and academia have also made ML and AI a contemporary priority.




\begin{figure}
  \centering
    \caption{ A typical machine learning process usually begins with a business or research need. An organization's leadership team launches a product or service, and customers start interacting with it. Additionally, domain experts are appointed to dig deeper into product research and analyze customer behavior. The domain experts may deploy additional sensors and conduct experiments to closely monitor different components of the system. All of these transactions, customer interactions, experiments and sensors produce a huge amount of data every day. It is impossible for the domain experts to manually mine knowledge and insights from all of this data --- this is where the data scientists come in. The data scientist first needs to clearly understand the data and the prediction goals from the domain experts. Then, the data scientist formulates computational prediction problems, extracts useful features from raw data, and selects a relevant ML model to solve the prediction problem. Once all these steps are done, existing AutoML models can be readily deployed to train and test the learning outcome as well as draw valuable insights from the data. The data scientist then reports back to the domain experts and business leaders with these results and communicates the most interesting findings. Based on these insights, the domain experts and business leaders make informed decisions to improve the product and address any existing issues with the system.}
    \label{fig:pipeline}
    
    \includegraphics[width=0.8\textwidth]{figures/EcoSystem.pdf}

\end{figure}


Although the ultimate goal of machine learning (ML) is to automatically draw conclusions from data and automate many of our tasks, developing ML solutions currently involves a lot of manual work by humans. \cz{As a result, many important steps of the ML process today are still done manually by the data scientist or ML engineer on an ad-hoc basis, including understanding the attributes of domain-specific data, formulating the definition of prediction problems, creating a suitable training data set, selecting a promising learning algorithm, and more. To reduce manual effort and thus accelerate deployment of machine learning technologies in practice, effort has been made to develop systems that attempted to help reducing the work in some steps of the whole workflow of developing a machine learning application. For example, DeepDive/Snorkel, is a general high-level workflow support system that can help users label and manage training data as well as provide high-level support for model selection. \cz{You can add some additional citations here if any}; such high-level support available in this kind of ``workflow support system," however, is at the cost of sacrificing the flexibility (e.g., in customizing the ML algorithms used). Another kind of systems aims to provide maximum flexibility by providing general and flexible support at a relatively lower level. For example, Google, Amazon and Microsoft have all provide cloud-based support of many ML capabilities via cloud-based services, and  a significant amount of research endeavor towards building AutoML systems in the past decade has resulted in hundreds of AutoML libraries/systems. ({\bf We need to explain what is AutoML}) However, all the existing systems have assumed that an ML problem has already been well defined by their users, but in practice, the very first step of identifying a promising opportunity of ML in a domain is quite challenging and time consuming. Once this time-consuming step is done, current AutoML systems mostly take care of \emph{Automated Feature Construction} and \emph{Hyper-parameter Tuning} steps of the whole machine learning pipeline. A typical process as it is practiced today is shown in Figure~\ref{fig:pipeline}.} This process also requires a lot of back-and-forth communication between data scientists and domain experts for clearly defining the prediction tasks and exploring alternative prediction opportunities, making the process difficult and inefficient. Several formative examples of such manual operations and lengthy back-and-forth interaction are presented in Table~\ref{table:scenario}. In many cases, it is unclear from the start what the data set can be used for, what predictions can be made and what other tasks can be formulated. Domain experts may want to change the problem definition after seeing first-round results, demanding a modification of the whole pipeline from scratch and thus further slowing down the process.




\begin{table*}

\caption{ Formative scenarios of manual operation and cross-functional interaction in  machine learning application for predictive modeling}
\label{table:scenario}

\renewcommand{\arraystretch}{0.2}
\begin{tabular}{p{13cm}}\\\hline
\begin{exmp}
A hospital collects patient electroencephalography (EEG) results on a regular basis, and wants to use them to predict which patients are most at risk for epilepsy. Doctors are not experts for building such predictive models. So, a data scientist is assigned to help but he/she may not have enough medical knowledge to understand the EEG log data and define the prediction task rigorously. Indeed, defining the \emph{risk} for epilepsy requires significant domain knowledge and experience and alternative definitions are possible too. The data scientist must actively collaborate with doctors and lab technicians to accurately understand and model the patient log data and setup the prediction task accordingly. In case of alternative definitions, multiple prediction tasks need to be defined and executed to address the need of the hospital / doctors.
\end{exmp}\\\hline

\begin{exmp}
A railway company continuously monitors signals from different engine sensors and wants to be able to predict the future failure of engine components. A data scientist working on this problem must collaborate with domain experts, including engineers, programmers, and even conductors, to fully understand the definition of failures and create effective training examples for learning an effective predictive model. The data scientist also needs to understand which hyper-parameters are involved in the definition and what is their acceptable range of values, in order to materialize the actual machine learning pipeline.
\end{exmp}\\\hline

\begin{exmp}
A wind energy company owns a number of huge turbines, each equipped with many sensors. Being able to predict turbine failure in advance can save headaches and reduce costs to the company. However, the numbers generated by the sensors are only meaningful to wind energy experts, so a data scientist working on this problem must spend long hours with them in order to understand the sensor data as well as the definition of turbine failure. Can any kind of stoppage be considered a turbine failure? Or, is there a particular threshold for time-range before the stoppage can be labeled as a failure? How soon a future failure needs to be identified? All these are important questions to answer before a concrete predictive task can be defined and executed thereby.
\end{exmp}\\\hline
\end{tabular}
\end{table*}


How can we make the current machine learning process more efficient and automated? How can we relieve the communication bottleneck between data scientists and domain experts? One option is to enable the domain experts to work with big data directly, without worrying about the underlying detailed knowledge of machine learning. Although this is a highly ambitious goal, if reached, it would expedite the implementation of machine learning systems allowing ML to appeal to a far broader audience. Imagine an intelligent agent that can guide domain experts in big data exploration and analytics tasks. In other words, think about a Virtual Interactive Data Scientist, which can perform many of the routine tasks performed by a \emph{Human} Data Scientist. Such a system would make big data analytics more appealing and accessible to business entities across various domains. At the same time, such system would increase the productivity of a human data scientist significantly by automating a big portion of their manual labor. 

In this paper, we lay out our vision for a Virtual Interactive Data Scientist (VIDS) to transform the current AutoML practice into a much faster and convenient alternate paradigm. VIDS can be thought of as an intelligent agent which, given a big corpus of data, starts talking to the domain experts in the language of a human data scientist in order to quickly figure out the user's need and explore alternative prediction opportunities. It can automatically come up with different prediction tasks, as well as explore multiple alternative learning models to solve the tasks. Based on these analyses, VIDS can then recommend useful tasks to the domain experts for further interpretation. Thus, a crucial design component of VIDS is human-computer interaction with a primary focus on user-friendly human-AI communication and human-oriented evaluation.

In summary, the primary features and benefits of VIDS, if materialized, can be summarized as follows:

\begin{enumerate}
    \item VIDS will communicate with users like a human data scientist and quickly understand their needs. It will translate these needs into well-defined prediction tasks.
    
    \item VIDS will propose different useful prediction tasks to the user simply by skimming through the data and improve these recommendations by communicating with users over multiple iterations.
    
    \item In parallel to proposing different prediction tasks, VIDS will also deploy alternative AutoML models for each prediction task and report the evaluation metric corresponding of the user's interest.
    
    \item VIDS will enable end-users to interactively play with infinite combinations of different prediction tasks and AutoML models by tweaking a minimal number of hyper-parameters and task preferences.
    
\end{enumerate}

%The rest of the paper is organized as follows: Section~\ref{sec:functions} discusses the core functions that data scientists currently perform. Section~\ref{sec:sota} reviews the state-of-the-art of machine learning literature corresponding to the \numberofessentialfunctions essential functions of data science, as well as the gaps and limitations in the current process. Section~\ref{sec:VIDS} describes the overall architecture of VIDS to address these limitations and then discusses each component in greater detail. Section~\ref{sec:Challenges} highlights the major challenges involved in realizing VIDS. Finally, Section~\ref{sec:conclusion} concludes the paper by discussing the potential impact of VIDS and possible future research directions in this area.


==> VDS.tex <==



\section{Virtual Interactive Data Scientist}\label{sec:VIDS}

\begin{figure*}
  \centering
    \caption{ This figure portrays a very high level overview of \emph{Virtual Interactive Data Scientist (VIDS)} architecture. The process starts with generating all possible prediction tasks by combining different target entities, constraint attributes and task-flow operators. $N$ denotes the total number of all possible prediction task. The next step in VIDS is to filter out $M$ (a user defined parameter) promising tasks out of the $N$ tasks, where $N \ggg M$, so that we don't have to execute the actual AutoML pipline for all $N$ tasks which is computationally very expensive. This filtering done based on metrics like \emph{User Preference}, \emph{Task Validity}, \emph{Business Potential Value} and \emph{Availability of  Sufficient Training Examples}. Next, the filtered top $M$ tasks are sent to the AutoML box which computes new metrics for the prediction tasks including \emph{Prediciton Accuracy}, \emph{Computation Time}, \emph{Confidence Interval}, \emph{Explanation of Model and Features} etc. As the AutoML pipeline completes, all the metrics for each promising prediction task are stored in a \emph{Prediction Task Metric Store}. Finally, these metric vector representations of $M$ promising tasks are fed to an ultimate recommender module, which outputs a ranked list of top $K$ tasks to the user.} 
    \label{fig:VIDS}
    
    \includegraphics[width=\linewidth]{figures/Model.pdf}
\end{figure*}


Our vision for Virtual Interactive Data Scientist (VIDS) is an intelligent agent that can formulate different prediction tasks and automatically recommend the best ones to its users. We envision VIDS as a more complete data science paradigm which considers any existing AutoML system as a blackbox and adds an interactive task generation and recommendation layer built on top of it. From the utility perspective, VIDS is a prediction task recommender system, which suggests useful prediction tasks to domain experts or business leaders and enables them to directly interact with the underlying world of Big Data. \medit{Computationally, VIDS takes \emph{Big Data} as input and outputs a set of recommended prediction tasks in an interactive fashion.}{Recommend deleting this sentence} The motivation for designing an interactive agent is also supported by \cite{yang2018grounding} where the authors investigated how non-experts (in machine learning) can build ML solutions for themselves in real life. Their empirical findings suggested that the interactive process of building ML models may lead to non-experts' greater trust in the learning results.


\subsection{The New Paradigm} 

Figure~\ref{fig:VIDS} provides a visual representation of VIDS's overall architecture. First, VIDS generates different prediction tasks by analyzing the given data set through a task-definition language. The task-definition language is composed of target entities, constraint attributes and task-flow operators (More details on task-definition language can be found in section~\ref{sec:PTG}.) Next, all tasks are passed to a task filter, which filters out any task which appears to be not useful before we waste AutoML resources on them.  Note that the ``utility" of a particular task heavily depends on the opinion of the end user, who in this case is a domain expert or business leader; thus, learning the right utility function is another job of VIDS. Some example metric for utility before running the AutoML include \emph{User Preference}, \emph{Task Validity}, \emph{Business Potential Value} and \emph{Availability of  Sufficient Training Examples}. Given a rigorous definition for these metrics, the task filter outputs the top $M$ tasks, where $N \ggg M$, which we call \emph{promising tasks}.

Next, each promising task is fed to an existing black box AutoML system where they go through the time-consuming steps of feature engineering, model selection, training and hyperparameter tuning. The AutoML module produces additional metrics for each prediction tasks like \emph{Prediciton Accuracy}, \emph{Computation Time}, \emph{Confidence Interval}, \emph{Explanation of Model and Features}. As soon as these steps are finished for each prediction task, its corresponding metrics are stored into a Prediction Task Metric Store. Finally, these metric vector representations of $M$ promising tasks are fed to an ultimate recommender module, which outputs the top $K$ tasks to the user along with their corresponding metric scores.


We defer to the user how they want to use this recommendation for their own benefit and/or interest. However, users may also give interactive feedback by marking some recommended tasks as useful and some as not-useful --- based on this feedback, VIDS can further refine its ranking function used for recommendation. If necessary, this refinement loop can continue over multiple iterations until the user is satisfied with the recommendations. 



\subsection{Breaking it into pieces} 
The twin core technical challenges in designing VIDS are to define a prediction task and evaluate its usefulness. In other words, realization of VIDS essentially boils down to the design of three complementary components shown in Figure~\ref{fig:VIDS}, which we discuss in more detail below.

\begin{enumerate}[leftmargin=*]
    \item {\bf Prediction Task Generation (PTG):} How can VIDS automatically generate a prediction task? To answer this question, we need a formal way to represent a prediction task, \eg a task definition language, and then, generate tasks using that representation. We formally define Prediction Task Generation as follows:

    \begin{defn}[Prediction Task Generation]\label{def:prediction-task-generation}
    Given a dataset $D$ with attribute set $S$ and general language $L$ to represent a family of prediction tasks, generate all possible prediction problems $T$ on $D$ \medit{using language $L$}{that can be expressed in language $L$}.
    \end{defn}



    \item {\bf Promising Task Selection (PTS):} How can VIDS identify a short list of promising tasks from an exponential number of tasks from the initial pool? This requires VIDS to automatically filter out invalid as well as uninteresting (user-dependent) tasks. Thus, defining \emph{validity}, \emph{user preference} etc. rigorously is crucial for effective implementation of PTS component, which would help VIDS for conducting an initial screening of the prediction tasks.

    \begin{defn}[Promising Task Selection]\label{def:promise}
    Given the set of all prediction tasks $T = \{t\}$, a user defined parameter $M$ and formal definitions of the following five functions:
    
    \[\text{Task Validity, } f_{v}(t): t \rightarrow \mathbb{R}\]
    \[\text{User Preference, } f_p(t) : t \rightarrow \mathbb{R}\]
    \[\text{Potential Business Value, } f_b(t) : t \rightarrow \mathbb{R}\]
    \[\text{Sufficient Training Examples, } f_e(t) : t \rightarrow \mathbb{R}\]
    
    \[\text{Promise, } \mathscr{F}_{promise}(t)=\mathscr{F}\left(f_v(t), f_p(t), f_b(t),f_e(t)\right): t \rightarrow \mathbb{R},\]
    
    
    Rank the prediction tasks from set $T$, according to their descending promise scores, i.e., $\mathscr{F}_{promise}(t)$, and return the top $M$ tasks.
    \end{defn}


    \item {\bf Ultimate Recommendation (UTR):} How can VIDS measure the \emph{utility} of each promising prediction task and provide recommendations based on the utility score? How can the task recommender system be quickly optimized? The definition of \emph{utility} here is non-trivial and can be a combined function of a number of metrics, some of which are outputs from executing the AutoML module on the prediction task, and some of which are already available from the Promising Task Selection step. Below, we provide a formal definition of the Prediction Task Recommendation problem.

    \begin{defn}[Ultimate Recommendation]\label{def:prediction-task-recommendation}
    Given a dataset $D$ with attribute set $S$, where attributes can be either categorical or numerical; a family of promising prediction tasks $P$, where each $p\in P$ represents a separate promising prediction task and $|P|=M$; a user defined parameter $K$, where $K$ is a \medit{non-negative}{I think this should read "positive"? Is it possible that K=0?} integer and a task utility function defined as follows:
    
    \[\text{Prediction Accuracy, } f'_{a}(t): t \rightarrow \mathbb{R}\]
    \[\text{Computation Time, } f'_{\tau}(t): t \rightarrow \mathbb{R}\]
    \[\text{Confidence Interval, } f'_{c}(t): t \rightarrow \mathbb{R}\]
    \[\text{Explainability, } f'_{x}(t): t \rightarrow \mathbb{R}\]
    
    \[\text{utility, } \mathscr{F}_{utility}(t): t\rightarrow\mathbb{R}\]

    \begin{dmath*}
    \mathscr{F}_{utility}(t)=\mathscr{F}\left(f_v(t), f_p(t), f_b(t),f_e(t), f'_{a}(t), f'_{a}(\tau), f'_{a}(c), f'_{x}(t)\right)
    \end{dmath*}
    
    
    Rank the prediction tasks from set $T$, according to their descending utility scores, i.e., $\mathscr{F}_{utility}(t)$, and return the top $K$ tasks.
    
    \end{defn}
\end{enumerate}




==> latexmkrc <==
#################################
# Personal compilations options #
#################################

$ENV{'TZ'}='America/New_York';

$bibtex_use = 2;
$pdf_mode = 1;
$pdflatex = 'pdflatex --shell-escape -synctex=1 %O %S';
$pdflatex_silent_switch = '-interaction=nonstopmode';

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}

